Relevance-guided Neural Machine Translation

With the advent of the Transformer architecture, Neural Machine Translation (NMT) results have shown great improvement lately. However, results in low-resource conditions still lag behind in both bilingual and multilingual setups, due to the limited amount of available monolingual and/or parallel data; hence, the need for methods addressing data scarcity in an efficient, and explainable way, is eminent. We propose an explainability-based training approach for NMT, applied in Unsupervised and Supervised model training, for translation of three languages of varying resources, French, Gujarati, Kazakh, to and from English. Our results show our method can be promising, particularly when training in low-resource conditions, outperforming simple training baselines; though the improvement is marginal, it sets the ground for further exploration of the approach and the parameters, and its extension to other languages.

==> description.tex <==
\clearpage
\setlength\rotFPtop{242pt}
\begin{sidewaystable}[htbp]
%\begin{table*}[ht]
\small
\begin{tabular}{l  B lll|l|lll|l|lll|l|lll|l}
\toprule
&&& \textbf{en-fr} & &&  & \textbf{fr-en} & && & \textbf{en-gu} &&&& \textbf{gu-en} && \\\hline
Parameters' Set Values &  & v1 & v2 & v3 && v1 & v2 & v3 && v1 & v2    & v3 && v1 & v2    & v3 \\\hline\hline
22k  &  && &&&   &&&   &&&   & \\\hline
Regular MT &&&&&31.12 &&&&30.63   &&&&1.04   &&&&2.65 \\
Regular BT+AE+MT &  &&&&34.54 &&&&34.02  &&&&1.16   &&&&2.19 \\\hline
MT  &&29.9&24.67&30.24&30.12&26.79 &\textbf{30.52}&2&2.18&\textbf{2.19}&0.69&0.7 &\textbf{0.73} \\
BT+AE+MT &&30.01&28.62&\textbf{32.15}&29.94&29.87&\textbf{33.03}&0.76&\textbf{1.36}&0.89&0.71&\textbf{1.06}&0.67\\\hline\hline
1m  & &&&&&&&&&&&&\\\hline
Regular MT &&&&&41.25 &&&&41.33   &&&&-   &&&&- \\
Regular BT+AE+MT &  &&&&40.37 &&&&40.4  &&&&-   &&&&- \\\hline
MT & &\textbf{39.12}& 38.12&35.44 && \textbf{39.2}&38.43&36.04&-&-&-&-&-&-\\
BT+AE+MT & & \textbf{37.58}& 37.22& 36.89&& 37.66& \textbf{37.95}& 37.38&-&-&-&-&-&-\\\hline\hline
2.5m  &&&&&&&&&&&&   &\\\hline
Regular MT &&&&&40.46 &&&&40.71   &&&&-   &&&&- \\
Regular BT+AE+MT &  &&&&39.88 &&&&39.62  &&&&-   &&&&- \\\hline
MT &  &\textbf{39.06}&36.02  &35.57&&\textbf{39.11} &36.28&36.09&-&-&-&-&-&-\\
BT+AE+MT &  &37.68 & 36.21& \textbf{37.74}  &&37.48 &36.66& \textbf{38.15}&-&-&-&-&-&-\\\hline\hline
5m &&&&&&&&&&&&&\\\hline
Regular MT &&&&&41.52 &&&&41.18   &&&&-   &&&&- \\
Regular BT+AE+MT &  &&&&40.89 &&&&40.8  &&&&-   &&&&- \\\hline
MT  &&\textbf{39.21} &37.55&39&&\textbf{39.33} &38.01&39.2&-&-&-&-&-&-\\
BT+AE+MT &&30.71&36.7&\textbf{37.48}&&32.02 &37.03&\textbf{37.67}&-&-&-&-&-&-
\end{tabular}
%\bottomrule
\hline
\caption{BLEU scores for Supervised, and Unsupervised + Supervised NMT Layerwise Relevance Propagation-guided experiments, for English - French, French - English, English - Gujarati, Gu - En. \emph{AE}, \emph{BT} and \emph{MT} stand for Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results_lrp_train}
\vspace{-0.5em}
%\end{table*}
\end{sidewaystable}

==> table_lrp_train_sideways.tex <==
\clearpage
\setlength\rotFPtop{242pt}
\begin{sidewaystable}[htbp]
%\begin{table*}[ht]
\small
\begin{tabular}{l  B lll|l|lll|l|lll|l|lll|l}
\toprule
&&& \textbf{en-fr} & &&  & \textbf{fr-en} & && & \textbf{en-gu} &&&& \textbf{gu-en} && \\\hline
Parameters' Set Values &  & v1 & v2 & v3 &Regular& v1 & v2 & v3 &Regular& v1 & v2    & v3 &Regular& v1 & v2    & v3&Regular \\\hline\hline
22k  &  && &&&   &&&   &&&   & \\\hline
%Regular MT &&&&&31.12 &&&&30.63   &&&&1.04   &&&&2.65 \\
%Regular BT+AE+MT &  &&&&34.54 &&&&34.02  &&&&1.16   &&&&2.19 \\\hline
MT  &&29.9&24.67&30.24&31.12&30.12&26.79 &\textbf{30.52}&30.63&2&2.18&\textbf{2.19}&1.04&0.69&0.7 &\textbf{0.73}&2.65 \\
BT+AE+MT &&30.01&28.62&\textbf{32.15}&34.54&29.94&29.87&\textbf{33.03}&34.02&0.76&\textbf{1.36}&0.89&1.16 &0.71&\textbf{1.06}&0.67&2.19\\\hline\hline
1m  & &&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.25 &&&&41.33   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.37 &&&&40.4  &&&&-   &&&&- \\\hline
MT & &\textbf{39.12}& 38.12&35.44 &41.25& \textbf{39.2}&38.43&36.04&41.33&-&-&-&-&-&-&-&-\\
BT+AE+MT & & \textbf{37.58}& 37.22& 36.89&40.37& 37.66& \textbf{37.95}& 37.38&40.4&-&-&-&-&-&-&-&-\\\hline\hline
2.5m  &&&&&&&&&&&&   &\\\hline
%Regular MT &&&&&40.46 &&&&40.71   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&39.88 &&&&39.62  &&&&-   &&&&- \\\hline
MT &  &\textbf{39.06}&36.02  &35.57&40.46&\textbf{39.11} &36.28&36.09&40.71&-&-&-&-&-&-&-&-\\
BT+AE+MT &  &37.68 & 36.21& \textbf{37.74} &39.88&40.71&37.48 &36.66& \textbf{38.15}&-&-&-&-&-&-&-&-\\\hline\hline
5m &&&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.52 &&&&41.18   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.89 &&&&40.8  &&&&-   &&&&- \\\hline
MT  &&\textbf{39.21} &37.55&39&41.52&\textbf{39.33} &38.01&39.2&41.18&-&-&-&-&-&-&-&-\\
BT+AE+MT &&30.71&36.7&\textbf{37.48}&40.89&32.02 &37.03&\textbf{37.67}&40.8&-&-&-&-&-&-&-&-
\end{tabular}
%\bottomrule
\hline
\caption{BLEU scores for Supervised, and Unsupervised + Supervised NMT Layerwise Relevance Propagation-guided experiments, for En - Fr, Fr - En, En - Gu, Gu - En. \emph{AE}, \emph{BT} and \emph{MT} stand for Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results_lrp_train}
\vspace{-0.5em}
%\end{table*}
\end{sidewaystable}

==> table_original.tex <==
\begin{table*}[ht]
\tiny
\begin{tabular}{lB lll|l|lll|l|lll|l|lll|l}
\toprule
&&& \textbf{en-fr} & &&  & \textbf{fr-en} & && & \textbf{en-gu} &&&& \textbf{gu-en} && \\\hline
Parameters' Set Values &  & v1 & v2 & v3 &Regular& v1 & v2 & v3 &Regular& v1 & v2    & v3 &Regular& v1 & v2    & v3&Regular \\\hline\hline
22k  &  && &&&   &&&   &&&   & \\\hline
%Regular MT &&&&&31.12 &&&&30.63   &&&&1.04   &&&&2.65 \\
%Regular BT+AE+MT &  &&&&34.54 &&&&34.02  &&&&1.16   &&&&2.19 \\\hline
MT  &&29.9&24.67&30.24&31.12&30.12&26.79 &\textbf{30.52}&30.63&2&2.18&\textbf{2.19}&1.04&0.69&0.7 &\textbf{0.73}&2.65 \\
BT+AE+MT &&30.01&28.62&\textbf{32.15}&34.54&29.94&29.87&\textbf{33.03}&34.02&0.76&\textbf{1.36}&0.89&1.16 &0.71&\textbf{1.06}&0.67&2.19\\\hline\hline
1m  & &&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.25 &&&&41.33   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.37 &&&&40.4  &&&&-   &&&&- \\\hline
MT & &\textbf{39.12}& 38.12&35.44 &41.25& \textbf{39.2}&38.43&36.04&41.33&-&-&-&-&-&-&-&-\\
BT+AE+MT & & \textbf{37.58}& 37.22& 36.89&40.37& 37.66& \textbf{37.95}& 37.38&40.4&-&-&-&-&-&-&-&-\\\hline\hline
2.5m  &&&&&&&&&&&&   &\\\hline
%Regular MT &&&&&40.46 &&&&40.71   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&39.88 &&&&39.62  &&&&-   &&&&- \\\hline
MT &  &\textbf{39.06}&36.02  &35.57&40.46&\textbf{39.11} &36.28&36.09&40.71&-&-&-&-&-&-&-&-\\
BT+AE+MT &  &37.68 & 36.21& \textbf{37.74} &39.88&40.71&37.48 &36.66& \textbf{38.15}&-&-&-&-&-&-&-&-\\\hline\hline
5m &&&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.52 &&&&41.18   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.89 &&&&40.8  &&&&-   &&&&- \\\hline
MT  &&\textbf{39.21} &37.55&39&41.52&\textbf{39.33} &38.01&39.2&41.18&-&-&-&-&-&-&-&-\\
BT+AE+MT &&30.71&36.7&\textbf{37.48}&40.89&32.02 &37.03&\textbf{37.67}&40.8&-&-&-&-&-&-&-&-
\end{tabular}
%\bottomrule
\hline
\caption{BLEU scores for Supervised, and Unsupervised + Supervised NMT Layerwise Relevance Propagation-guided experiments, for En--Fr, Fr--En, En--Gu, Gu--En. \emph{AE}, \emph{BT} and \emph{MT} stand for Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results_lrp_train_fr_gu}
\vspace{-0.5em}
\end{table*}

==> table_res.tex <==
\begin{table}[ht]
\small
\centering
%\resizebox{\textwidth}{}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Method}  & \textbf{en-fr}  & \textbf{fr-en} &\textbf{En - Gu} & \textbf{Gu - En}  \\ 
\hline
\multicolumn{4}{l}{\emph{Other methods}} \\ \hline
other &  &  &  &  \\
\hline
\multicolumn{4}{l}{\emph{Ours}} \\ \hline\hline
BT+AE    &21.76   &21.69&0.35  &0.4  \\ \hline
22k&&&\\\hline\hline
MT    & 34.54  & 34.02& \textbf{2.43} &\textbf{1.04} \\ 
BT+AE+MT  & 30.09  & 30.07& 1.32 & 1.04 \\ \hline
1m&&&\\\hline\hline
MT   &42.07&41.68& - & -  \\
BT+AE+MT   &42.1&41.85& - & - \\\hline
2.5m&&&&\\\hline\hline
MT   &42.15&41.68& - & -  \\
BT+AE+MT   &\textbf{42.47}&\textbf{42.02}& - & - \\\hline
5m&&&&\\\hline\hline
MT   & 41.75  & 41.41& - & -  \\ 
BT+AE+MT   & 40.89  & 40.8& - & -
\end{tabular}
%\vspace*{-0.5em}
\bottomrule
\vspace*{0.5em}
\caption{BLEU scores for Unsupervised, Supervised, and Unsupervised + Supervised NMT experiments, for En - Gu, Gu - En, en-fr, fr-en. \emph{AE}, \emph{BT} and \emph{MT} stand for Masked Language Model, Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results}
\vspace{-0.5em}
\end{table}

%\include{table_res}

==> train_lrp_gu.tex <==

%\begin{sidewaystable}[htbp]
\begin{table*}[ht]
\tiny
\begin{tabular}{lB lll|l|lll|l}
\toprule
&& & \textbf{en-gu} &&&& \textbf{gu-en} && \\\hline
Parameters' Set Values &  & v1 & v2 & v3 &Regular& v1 & v2 & v3 &Regular \\\hline\hline
22k &&&&& \\\hline
%Regular MT &&&&&31.12 &&&&30.63   &&&&1.04   &&&&2.65 \\
%Regular BT+AE+MT &  &&&&34.54 &&&&34.02  &&&&1.16   &&&&2.19 \\\hline
MT  &&2&2.18&\textbf{2.19}&1.04&0.69&0.7 &\textbf{0.73}&2.65 \\
BT+AE+MT &&0.76&\textbf{1.36}&0.89&1.16 &0.71&\textbf{1.06}&0.67&2.19\\\hline\hline
1m  & &&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.25 &&&&41.33   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.37 &&&&40.4  &&&&-   &&&&- \\\hline
MT & &-&-&-&-&-&-&-&-\\
BT+AE+MT & &-&-&-&-&-&-&-&-\\\hline\hline
2.5m  &&&&   &\\\hline
%Regular MT &&&&&40.46 &&&&40.71   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&39.88 &&&&39.62  &&&&-   &&&&- \\\hline
MT &  &-&-&-&-&-&-&-&-\\
BT+AE+MT &  &-&-&-&-&-&-&-&-\\\hline\hline
5m &&&&&\\\hline
%Regular MT &&&&&41.52 &&&&41.18   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.89 &&&&40.8  &&&&-   &&&&- \\\hline
MT  &&-&-&-&-&-&-&-&-\\
BT+AE+MT &&-&-&-&-&-&-&-&-
\end{tabular}
%\bottomrule
\hline
\caption{BLEU scores for Supervised, and Unsupervised + Supervised NMT Layerwise Relevance Propagation-guided experiments, for En--Gu, Gu--En. \emph{AE}, \emph{BT} and \emph{MT} stand for Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results_lrp_gu}
\vspace{-0.5em}
\end{table*}
%\end{sidewaystable}

==> train_lrp_train.tex <==

%\begin{sidewaystable}[htbp]
\begin{table*}[ht]
\tiny
\begin{tabular}{lB lll|l|lll|l|lll|l|lll|l}
\toprule
&&& \textbf{en-fr} & &&  & \textbf{fr-en} & && & \textbf{en-gu} &&&& \textbf{gu-en} && \\\hline
Parameters' Set Values &  & v1 & v2 & v3 &Regular& v1 & v2 & v3 &Regular& v1 & v2    & v3 &Regular& v1 & v2    & v3&Regular \\\hline\hline
22k  &  && &&&   &&&   &&&   & \\\hline
%Regular MT &&&&&31.12 &&&&30.63   &&&&1.04   &&&&2.65 \\
%Regular BT+AE+MT &  &&&&34.54 &&&&34.02  &&&&1.16   &&&&2.19 \\\hline
MT  &&29.9&24.67&30.24&31.12&30.12&26.79 &\textbf{30.52}&30.63&2&2.18&\textbf{2.19}&1.04&0.69&0.7 &\textbf{0.73}&2.65 \\
BT+AE+MT &&30.01&28.62&\textbf{32.15}&34.54&29.94&29.87&\textbf{33.03}&34.02&0.76&\textbf{1.36}&0.89&1.16 &0.71&\textbf{1.06}&0.67&2.19\\\hline\hline
1m  & &&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.25 &&&&41.33   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.37 &&&&40.4  &&&&-   &&&&- \\\hline
MT & &\textbf{39.12}& 38.12&35.44 &41.25& \textbf{39.2}&38.43&36.04&41.33&-&-&-&-&-&-&-&-\\
BT+AE+MT & & \textbf{37.58}& 37.22& 36.89&40.37& 37.66& \textbf{37.95}& 37.38&40.4&-&-&-&-&-&-&-&-\\\hline\hline
2.5m  &&&&&&&&&&&&   &\\\hline
%Regular MT &&&&&40.46 &&&&40.71   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&39.88 &&&&39.62  &&&&-   &&&&- \\\hline
MT &  &\textbf{39.06}&36.02  &35.57&40.46&\textbf{39.11} &36.28&36.09&40.71&-&-&-&-&-&-&-&-\\
BT+AE+MT &  &37.68 & 36.21& \textbf{37.74} &39.88&40.71&37.48 &36.66& \textbf{38.15}&-&-&-&-&-&-&-&-\\\hline\hline
5m &&&&&&&&&&&&&\\\hline
%Regular MT &&&&&41.52 &&&&41.18   &&&&-   &&&&- \\
%Regular BT+AE+MT &  &&&&40.89 &&&&40.8  &&&&-   &&&&- \\\hline
MT  &&\textbf{39.21} &37.55&39&41.52&\textbf{39.33} &38.01&39.2&41.18&-&-&-&-&-&-&-&-\\
BT+AE+MT &&30.71&36.7&\textbf{37.48}&40.89&32.02 &37.03&\textbf{37.67}&40.8&-&-&-&-&-&-&-&-
\end{tabular}
%\bottomrule
\hline
\caption{BLEU scores for Supervised, and Unsupervised + Supervised NMT Layerwise Relevance Propagation-guided experiments, for En--Fr, Fr--En, En--Gu, Gu--En, En--So, So--En. \emph{AE}, \emph{BT} and \emph{MT} stand for Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Test and validation sets are from WMT19 for Gujarati, and newstest2013-14 for French.}
\vspace{-2mm}
\label{table:bleu_results_lrp_train}
\vspace{-0.5em}
\end{table*}
%\end{sidewaystable}
